A Data-Driven Algorithm for Model-Free Control Synthesis

Presented is an algorithm to synthesize the optimal infinite-horizon LQR feedback controller for continuous-time systems. The algorithm does not require knowledge of the system dynamics but instead uses only a finite-length sampling of input-output data. A necessary condition that relates the optimal LQR gain to any arbitrary solution trajectory of the system is presented. An algorithm using this necessary condition, based on constrained optimization, is developed that estimates the LQR gain matrix. In addition to calculating the standard feedback gain matrix, a feedforward gain can be found to implement a reference tracking controller. This paper presents a theoretical justification for the method and shows several examples, including a validation test flight on a real scale aircraft with unknown dynamics.

==> Sections/results.tex <==
Two results cases will now be presented. First, the solution methodology is verified using a known linear system. Data is generated from the linear system and a controller is found by solving \eqref{eq:NLP}. We refer to the state feedback gain matrix computed by the proposed model-free method as $K_{\text{MF}}$. We then compare the model-free gain matrix to the one computed when $A$ and $B$ are known using a classical ARE approach. We denote this gain matrix as $K_\text{LQR}$. This comparison is illustrated in Figure \ref{fig:flowchart}.

Second, the model-free controller methods are applied to stabilize an unknown nonlinear system about an equilibrium point. This example demonstrates the versatility of the approach, especially on systems that are unknown, difficult to linearize, or have high dimensional state spaces. The gain matrix from the model-free approach is compared to the gain matrix using $A$ and $B$ generated by linearizing the known nonlinear model about the equilibrium point.

All simulation results have been implemented using MATLAB R2024a and Simulink.  For the optimization in \eqref{eq:NLP} we use the NLP code IPOPT \cite{wachter2006implementation}, where
the constraint Jacobian was computed using automatic differentiation by the methods of \cite{andersson2019casadi}. The NLP was initialized by setting $X = Y $, $L = I \in \Rnn$, and $S = {\mathbf{1}} \in \Rnm$.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/flowchart.jpg}
    \caption{The testing paradigm for Example 1.}
    \label{fig:flowchart}
\end{figure}

\subsection{Known Linear System} \label{sec:results linear}

Our first example is the fourth-order linearized model of the lateral-perturbation equations of motion for an aircraft \cite[Sec. 10.1.2, p. 148]{bryson1994control}. Coefficients for the model are found from \cite[Sec. IX, p. 210]{heffley1972aircraft} and represent a Boeing 747 traveling at 774 ft/s (Mach 0.8) at an altitude of 40,000 ft. The lateral state vector is defined as $x = \begin{bmatrix} \beta & r & p & \phi \end{bmatrix}^\top$, where the state elements are sideslip angle, yaw rate, roll rate, and roll angle, respectively. The input is the rudder deflection, $u = \delta r$, and the model is as follows:
\begin{equation}
\begin{aligned}
        \dot x = & \begin{bmatrix}
            -0.0558 & -0.9968 & 0.0802 & 0.0415 \\
            0.598 & -0.115 & -0.0318 & 0\\
            -3.05 & 0.388 & -0.4650 & 0\\
            0 & 0.0805 & 1 & 0\end{bmatrix}x \\ & + \begin{bmatrix} 0.00729 \\ -0.475 \\ 0.153 \\ 0 \end{bmatrix}u.
        \label{eq:747latsys}
\end{aligned}
\end{equation}
 The data for this example was generated by choosing for the input sequence a linear-frequency chirp, defined as
 $u_k= \psi \sin \lp 2\pi\lp \frac{c}{2} t_k^2 + f_0t_k \rp \rp$, where $\psi =1\mathrm{e}-4$, $f_0 = 1\mathrm{e}-4$, $f_1 = 7\mathrm{e}-2$, and $c = \lp f_1 - f_0 \rp / T$.

The data collected was sampled at 10 Hz for $T=30$ seconds. The generation of $y_k$ included a small amount of standard normal Gaussian random noise added to the signal to mimic sensor noise. The pair $\lp y_k, u_k \rp$ along with user defined LQR weighting matrices, $M = \text{diag}[\begin{matrix}10&1&1&10\end{matrix}]$ and $R = I$, are the inputs to the optimization problem \eqref{eq:NLP}. The optimal closed-loop controller matrix was computed as
\begin{equation}\label{eq:747Kopt}
    K_\text{MF} = \begin{bmatrix} 9.2236 & -6.6657 & -3.1473 & -2.9555\end{bmatrix}.
\end{equation}

Since the original linear system is known, the resulting LQR controller matrix, for the same $M$ and $R$, can be computed directly using MATLAB's LQR solver, which gives
\begin{equation}\label{eq:747Klqr}
    K_\text{LQR} = \begin{bmatrix} 9.3477 & -7.4703 & -3.3029 & -2.9165\end{bmatrix}.
\end{equation}

Comparing \eqref{eq:747Kopt} and \eqref{eq:747Klqr} shows nearly identical resulting controllers. Some small deviation from the ground-truth optimal controller is expected due to the presence of noise in the data, $y_k$, as well as the fact a finite difference approximation was used in \eqref{eq:finte diff in V}.

The closed-loop response of the system with each controller was simulated. Figure \ref{fig:747_roll_tracking} illustrates the system response to a $\pm 10^\circ$ roll doublet input. The command tracking performance of the model-free controller closely resembles the performance of the ground-truth LQR controller.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/747_roll_tracking.eps}
    \caption{The state response after implementation of a B-747 roll command tracking. The ground truth is generated with $K_{LQR}$ and is shown with the dashed red line. The response when using the controller, $K_{MF}$, computed with the proposed model-free method is shown in blue. Best viewed in color.}
    \label{fig:747_roll_tracking}
\end{figure}

\subsection{Unknown Nonlinear System} \label{sec:results nonlinear}

As a second example, we select a problem of controlling a real-world flight vehicle by utilizing the presented model-free control approach. This process can be used in conjunction with a flight test program to refine vehicle flight performance characteristics that would be unknown or uncertain in the initial design phases.

A high-fidelity nonlinear model of an Holybro X500 V2 quadcopter was implemented in Simulink featuring six-degree-of-freedom (6DOF) equations of motion, electronic speed control (ESC) dynamics, real-world motor and propeller aerodynamic data \cite{tyto1580}, and a FlightGear graphical interface with a joystick input for manual pilot commands. Using a high-fidelity simulation to generate the data was chosen so as to compare the resulting controller to the ground-truth.

The X500-V2 is an X-configuration quadcopter whose motors are labeled 1-4 beginning with the front left motor and counting clockwise. A diagram of the airframe can be seen in Figure \ref{fig:Quad}.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Quad_Dimensions.pdf}
    \caption{The depiction of the body coordinate frame and dimensions of the Holybro X500 V2 quadcopter for which the Simulink model used for example 2 in Section \ref{sec:results nonlinear} is based on.}
    \label{fig:Quad}
\end{figure}

This simulation uses a Flat-Earth inertial reference frame, $e$, whose principal axis extend in the north-east-down (NED) directions. Additionally, the body-fixed axis, $b$, is defined with the \textit{x}-direction aligned with a vector pointing forward between motors 1 and 2, \textit{y}-direction pointing to the right of the frame between motors 2 and 3, and \textit{z}-direction pointing downward, completing the triad whose origin is at the center of gravity of the body. The twelve states tracked in the simulation are the inertial NED position, $P_e = [\begin{matrix} p_n & p_e & p_d\end{matrix}]^\top$, Euler orientation angles, $\Phi = [\begin{matrix} \phi & \theta & \psi \end{matrix}]^\top$, body-fixed velocity, $V_b = [\begin{matrix} u_b & v_b & w_b\end{matrix}]^\top$, and angular velocity of body $b$ with respect to the inertial frame $e$, $\omega_{b/e} = [\begin{matrix} p & q & r \end{matrix}]^\top$. The translational equations of motion of the quadcopter are given by
\begin{equation}
\begin{cases}
            \begin{aligned}
                \dot P_e & = C_{b/e}(\Phi) V_b\\
                \dot V_b & = \frac{1}{m}F_b - \omega_{b/e} \times V_b,
            \end{aligned}
        \label{eq:6dof trans}
    \end{cases}
\end{equation}
where $C_{b/e}(\Phi)$ is the 3-2-1 Euler rotation matrix from $b$ to $e$. The total external force vector can separated into individual gravity, drag, and propulsive force contributions as
\begin{equation}
\begin{aligned}
        F_b & =  F_{gravity} + F_{drag} + F_{propulsion}.\\
        \end{aligned}
        \end{equation}
 For the quadcopter, these components can be expressed as
\begin{equation}
    \begin{aligned}
        F_b &  = C_{e/b}(\Phi)\begin{bmatrix}
        0\\ 0\\ mg
    \end{bmatrix} + \begin{bmatrix}
        F_{drag,x}\\
        F_{drag,y}\\
        F_{drag,z}\\
    \end{bmatrix} + \begin{bmatrix}
        0\\ 0\\ -T
    \end{bmatrix}.
    \end{aligned}
\label{eq:F_b}
\end{equation}
% Only drag force is included in the aerodynamic forces since any lift force generated by the body is negligible and the primary lift is generated by the thrust of the propulsion system. 
Each of the drag force components can be computed using information from the drag coefficient $C_d$, a reference area, $S$, and the air density, $\rho$. For example, in the x-direction we have, $F_{drag,x} = - \text{sign}(u_b) \times 1/2\rho u_b^2 \times S_x \times C_{d,x}$. The rotational equations of motion of the quadcopter are given by
\begin{equation}
    \begin{cases}
        \begin{aligned}
            \dot \Phi & = W\lp \Phi\rp \omega_{b/e}\\
            \dot \omega_{b/e} & = I_b^{-1} \left[ M_b - \omega_{b/e} \times \lp I_b \omega_{b/e} \rp \right],
        \end{aligned}
    \end{cases}
    \label{eq:6dof rot}
\end{equation}
where
\begin{equation}
    \begin{aligned}
        W (\Phi) = \begin{bmatrix}
                1 & \sin\phi\tan\theta & \cos\phi\tan\theta\\
                0 & \cos\phi & -\sin\phi\\
                0 & \sin\phi/\cos\theta & \cos\phi/\cos\theta
            \end{bmatrix} 
    \end{aligned}
\end{equation}
is the rotational kinematics matrix and $I_b$ is the moment of inertia matrix for the quadcopter. The applied moment vector can be expanded as
\begin{equation}
    \begin{aligned}
        M_b = \begin{bmatrix}
            M_x \\ M_y \\ M_z
        \end{bmatrix}
    \end{aligned}.
\end{equation}

The simulation was designed to be operated from user-inputs through a joystick yielding a  four dimensional control vector consisting of one throttle and three torque control inputs. The user commands a primary throttle setting, $\Gamma\in[0, 1]$, via a throttle lever, that corresponds to the desired altitude. Rotating the joystick produces three input signals, $\begin{bmatrix}\tau_\text{r} & \tau_\text{p} & \tau_\text{y} \end{bmatrix}^\top \in [-1, 1]$, that perturb the attitude of the quadcopter by specifically increasing or decreasing individual motor speeds to produce the desired body torque. In matrix form the mapping from joystick inputs to commanded motors speeds is
\begin{equation}
    \begin{aligned}
        \begin{bmatrix}
            w_{1,\text{cmd}} \\ w_{2,\text{cmd}}  \\ w_{3,\text{cmd}}  \\w_{4,\text{cmd}} 
        \end{bmatrix} = \begin{bmatrix}
            K_{\Gamma} & -K_{\text{r}} & K_{\text{p}} & K_{\text{y}} \\
            K_{\Gamma} &   K_{\text{r}} & K_{\text{p}} & -K_{\text{y}} \\
            K_{\Gamma} &   K_{\text{r}} & -K_{\text{p}} & K_{\text{y}} \\
            K_{\Gamma} & -K_{\text{r}} & -K_{\text{p}} & -K_{\text{y}} \\
        \end{bmatrix}
        \begin{bmatrix}
            \Gamma \\ \tau_{\text{r}} \\ \tau_{\text{p}} \\ \tau_{\text{y}}
        \end{bmatrix},
        \end{aligned}
\end{equation}
where a scalar gains $K_{\Gamma,\text{r},\text{p},\text{y}}>0$ are used to transform the joystick input signal to appropriate units. The commanded motor speed vector, $w = \begin{bmatrix} w_{1,\text{cmd}} & w_{2,\text{cmd}}  & w_{3,\text{cmd}}  & w_{4,\text{cmd}} \end{bmatrix}^\top $, forms the plant input signals.

Inside the plant model, electronic speed controller dynamics are modeled  to track the relationship between commanded motor speeds, $w_{i,\text{cmd}}$, to achieved motor speed, $w_{i,\text{ach}}$.  The total thrust $T = \sum_{i=1}^4 T_i$ is the sum of all individual motor thrusts, $T_i$, and the applied torques can be computed from motor thrusts as
\begin{equation}
    \begin{aligned}
        \begin{bmatrix}
            M_x \\ M_y
        \end{bmatrix} & = 
        \begin{bmatrix}
            -d\sqrt{2}/2 & d\sqrt{2}/2& d\sqrt{2}/2 & -d\sqrt{2}/2 \\ 
             d\sqrt{2}/2 & d\sqrt{2}/2& -d\sqrt{2}/2 & -d\sqrt{2}/2 \\ 
        \end{bmatrix}
        \begin{bmatrix}
            T_1\\ T_2\\ T_3\\ T_4
        \end{bmatrix}\\
        M_z & = M_1 - M_2 + M_3 - M_4.
    \end{aligned}
    \label{eq:control torques}
\end{equation}
Motor thrusts and moments, $T_i$ and $M_i$, were extracted from a lookup table of experimental data relating commanded motor speeds and the resulting thrust or torque value. The complete set of nonlinear dynamics, $\dot X = f(X,U)$, for the 6DOF model is given with \eqref{eq:6dof trans} and \eqref{eq:6dof rot} where the twelve dimensional vehicle state becomes $X = [\begin{matrix} P_e & V_b & \Phi & \omega_{b/e}\end{matrix}]^\top$. Interested readers should see \cite{stevens_aircraft_2015} for additional 6DOF modeling details. A simplified moment of inertia is calculated from $I^b = \text{diag}\begin{bmatrix}I_{xx} & I_{yy} & I_{zz}\end{bmatrix}$. Physical parameters for the X500 V2 are listed in Table \ref{tab:quad params}.

\begin{table}
\renewcommand{\arraystretch}{1.3}
\caption{\bf X500 V2 Quadcopter Parameters}
\label{tab:quad params}
\centering
\begin{tabular}{|c|c|c|}
\hline
\bfseries Parameter & \bfseries Value & \bfseries Units\\
\hline\hline
Mass, $m$              & 1.3269 & $kg$\\
X-inertia, $I_{xx}$& $0.01295$ & $kg\cdot m^2$\\
Y-inertia, $I_{yy}$& $0.01244$ & $kg\cdot m^2$\\
Z-inertia, $I_{zz}$& $0.01571$ & $kg\cdot m^2$\\
Arm Length, $d$        & 0.25   & $m$\\
Thrust Coefficient, $C_T$ & 3.1539e--5& $N\cdot s^2/rad^2$\\
Torque Coefficient, $C_Q$ & 4.3543e--9&  $N\cdot s^2/rad^2$\\
Min Motor Speed           & 115 & $rad/s$\\
Max Motor Speed           & 907 & $rad/s$\\
\hline
\end{tabular}
\end{table}
The goal is to compute an attitude controller to stabilize the roll and pitch dynamics. First, in-flight state data was recorded by using a pilot-operated joystick to input roll and pitch oscillations into the quadcopter dynamics. Figure \ref{fig:quad_pitchroll_inputs} presents the roll and pitch joystick inputs. These inputs are kept small in magnitude $\lp \pm 1^\circ \rp$ to maintain trajectories near the equilibrium point. Since the system is nonlinear, we expect the system to behave only approximately linearly in a neighborhood around the equilibrium point. By keeping the input small, we avoid a flight region where the response begins to deviate significantly from the approximately linear regime.

Note that while the control inputs in this example were generated manually from a human-operated joystick in an open-loop system, data could also be collected from vehicle using a sub-optimal closed-loop controller.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/quad_pitchroll_inputs.eps}
    \caption{Joystick generated manual control inputs, in the pitch(below) and roll (above) axes. }
    \label{fig:quad_pitchroll_inputs}
\end{figure}

Next, using the generated noisy state and input pair $\lp y_k, u_k \rp$, an optimal controller was computed for the weighting matrices $M = \text{diag}[\begin{matrix}100&100&1&1\end{matrix}]$ and $R = \text{diag}[\begin{matrix}0.1&0.1\end{matrix}]$. We reduce the dimensionality of the state space to only the attitude-related states and inputs for controller synthesis, that is, $x = \begin{bmatrix} \phi & \theta & p & q\end{bmatrix}^\top$ and $u = \begin{bmatrix} \tau_\text{roll} & \tau_\text{pitch}\end{bmatrix}^\top$. The optimal model-free closed loop controller was computed as
\begin{equation}\label{eq:quadKopt}
    K_\text{MF} = \begin{bmatrix} 31.8563 & 0 & 10.2369 & 0 \\
                                   0 & 31.5142 & 0 & 10.2665 \end{bmatrix}.
\end{equation}
The nonlinear quadcopter simulation was linearized about the hover trim condition, a linear system was extracted, and an LQR controller was computed. The LQR gain matrix was calculated as
\begin{equation}\label{eq:quadKlqr}
    K_\text{LQR} = \begin{bmatrix} 31.6228 & 0 & 10.2900 & 0 \\
                                   0 & 31.6228 & 0 & 10.0965 \end{bmatrix}.
\end{equation}
Again, notice the close resemblance between $K_\text{opt}$ and $K_\text{lqr}$, indicating that the model-free controller is approaching the optimal LQR solution.

The performance of each of the controllers was compared by simulating the nonlinear quadcopter closed-loop system. Figure \ref{fig:quad_pitchroll_tracking} shows the quadcopter response to simultaneous roll ($\pm 5^\circ$ at $1/2$Hz) and pitch ($\pm 12^\circ$ at $1/5$Hz) doublets. The command tracking performance of the model-free controller closely resembles the performance of the ground-truth LQR controller.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/quad_pitchroll_tracking.eps}
    \caption{The state response after implementation of an attitude command tracking on a quadcopter 
    drone. The ground truth is generated with $K_{LQR}$ and is shown with the dashed red line. The response when using the controller, $K_{MF}$, computed with the proposed model-free method is shown in blue. Best viewed in color.}
    \label{fig:quad_pitchroll_tracking}
\end{figure}
